Disentangling the magneto-optic Kerr effect of manganite epitaxial heterostructures

Magneto-optic Kerr effect can probe the process of magnetization reversal in ferromagnetic thin films and thus be used as an alternative to magnetometry. Kerr effect is wavelength-dependent and the Kerr rotation can reverse sign, vanishing at particular wavelengths. We investigate epitaxial heterostructures of ferromagnetic manganite, La$_{0.7}$Sr$_{0.3}$Mn$_{0.9}$Ru$_{0.1}$O$_3$, by polar Kerr effect and magnetometry. The manganite layers are separated by or interfaced with a layer of nickelate, NdNiO$_3$. Kerr rotation hysteresis loops of trilayers, with two manganite layers of different thickness separated by a nickelate layer, have intriguing humplike features, when measured with light of 400 nm wavelength. By investigating additional reference samples we disentangle the contributions of the individual layers to the loops: we show that the humps originate from the opposite sense of the Kerr rotation of the two different ferromagnetic layers, combined with the additive behavior of the Kerr signal.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
